RASMALAI: Resources for Adaptive Speech Modeling in Indian Languages with Accents and Intonations

We introduce RASMALAI, a large-scale speech dataset with rich text descriptions, designed to advance controllable and expressive text-to-speech (TTS) synthesis for 23 Indian languages and English. It comprises 13,000 hours of speech and 24 million text-description annotations with fine-grained attributes like speaker identity, accent, emotion, style, and background conditions. Using RASMALAI, we develop IndicParlerTTS, the first open-source, text-description-guided TTS for Indian languages. Systematic evaluation demonstrates its ability to generate high-quality speech for named speakers, reliably follow text descriptions and accurately synthesize specified attributes. Additionally, it effectively transfers expressive characteristics both within and across languages. IndicParlerTTS consistently achieves strong performance across these evaluations, setting a new standard for controllable multilingual expressive speech synthesis in Indian languages.

==> sections/3_methodology.tex <==
% \section{Methodology}
% % A key limitation of Parler-TTS in its original design is its reliance on a tokenizer that supports only the Latin script, making it unsuitable for Indian languages that use diverse and phonetically rich writing systems. To enable high-quality synthesis across these scripts, we extend the Llama2 tokenizer, ensuring strong fertility scores for Indian languages. Our approach follows the methodology described in~\cite{mundra2024empirical}, allowing for improved subword segmentation. We also add special tokens to model noise-tags in this tokenizer.


% \textbf{Write that we finetune on TTS datasets with named speakers.}
% % that better preserves linguistic structure while remaining efficient for TTS. 
% % \subsection{Tokenizer}
% % After replacing the prompt tokenizer, we reinitialize the embedding space of the Parler-TTS v1-mini model to accommodate the new token set. To ensure smooth adaptation, we employ a two-stage training process:
% % \begin{enumerate}
% %     \item \textbf{Warm-Up Phase:} The embedding layer is trained for 1000 steps with the rest of the model frozen. This allows the embedding space to align with the new token set while preserving the pre-trained knowledge of the rest of the model. 
% %     \item \textbf{Full Fine-Tuning:} All components of the model are unfrozen for end-to-end fine-tuning, optimizing performance on Indian languages.
% % \end{enumerate}

% % \subsection{Description Encoder}
% % The Flan-T5 large encoder is crucial for the Indic Parler TTS system as it effectively aligns synthesized speech with textual descriptions. By encoding complex descriptions into rich representations, it provides the TTS decoder with precise guidance, ensuring high-quality, contextually accurate speech generation. This alignment capability is key to achieving natural-sounding TTS with improved contextual fidelity.

% % \subsection{Neural Audio Codec}
% % The choice of the 44.1kHz Descript audio codec~\cite{} for Indic Parler TTS is primarily motivated by its computational efficiency. Unlike the 24kHz version, which uses 32 residual quantizers, the 44.1kHz model employs only 8, significantly reducing computational overhead. This reduction in quantizers allows for faster processing without compromising audio quality, making the 44.1kHz codec a more scalable and efficient option for high-performance, real-time speech synthesis

% % \subsection{Delayed Pattern Prediction}
% % % \textbf{Rewrite as we follow MusicGen's delayed pattern prediction.}
% % Delayed Pattern Prediction enhances the prediction of discrete units in RVQ-GAN models by leveraging the hierarchical structure of residual codebooks. Each successive codebook captures increasingly finer-grained details, and this approach enforces a delay between the predictions of higher-order codebooks relative to lower-order ones.

% % \begin{enumerate}
% %     \item \textbf{Explicit Hierarchical Modeling:} Higher-order codebooks are conditioned on representations from lower-order ones, reinforcing the hierarchical dependencies inherent in RVQ-GAN.
% %     \item \textbf{Improved Contextual Representation:} The delayed prediction allows the model to utilize richer contextual information, improving its ability to capture complex phonetic and prosodic variations.
% % \end{enumerate}

